Guided Automated Learning for query workload re-Optimization

Query optimization is a hallmark of database systems enabling complex SQL queries of today's applications to be run efficiently. The query optimizer often fails to find the best plan, when logical subtleties in business queries and schemas circumvent it. When a query runs more expensively than is viable or warranted, determination of the performance issues is usually performed manually in consultation with experts through the analysis of query's execution plan (QEP). However, this is an excessively time consuming, human error-prone, and costly process. GALO is a novel system that automates this process. The tool automatically learns recurring problem patterns in query plans over workloads in an offline learning phase, to build a knowledge base of plan-rewrite remedies. It then uses the knowledge base online to re-optimize queries queued for execution to improve performance, often quite drastically. GALO's knowledge base is built on RDF and SPARQL, W3C graph database standards, which is well suited for manipulating and querying over SQL query plans, which are graphs themselves. GALO acts as a third-tier of re-optimization, after query rewrite and cost-based optimization, as a query plan rewrite. Since the knowledge base is not tied to the context of supplied QEPs, table and column names are matched automatically during the re-optimization phase. Thus, problem patterns learned over a particular query workload can be applied in other query workloads. GALO's knowledge base is also an invaluable tool for database experts to debug query performance issues by tracking to known issues and solutions as well as refining the optimizer with new tuned techniques by the development team. We demonstrate an experimental study of the effectiveness of our techniques over synthetic TPC-DS and real IBM client query workloads.

==> algorithms/CreateTemplate.tex <==
% Algorithm used to create a template for an array of RDFGs

%\paddingTopAlgorithm{}
\begin{algorithm}
  \caption{Generate template from RDFGs}
  \label{alg:createTemplate}
  \begin{algorithmic}[1]
    \Input{QEP files represented as RDF graphs, $RDFGs$[ ]}
    \Output{Template generated from the RDF graphs, $template$}
    \Function{generateTemplate}{ $RDFGs$[ ] }
      \ForEach{$resource$ in $RDFGs$}
        \State $lowProps$[ ] := find lowest value for each $prop$ in $resource$
        \State $highProps$[ ] := find highest value for $prop$ in $resource$
        \State $templateRes$ := generate a resource with $lowProps$[ ] and $highProps$[ ]
        \State $template$.add($resource$)
      \EndFor
      \State \Return{$template$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}
%\paddingBottomAlgorithm{}

==> algorithms/FindBestPlan.tex <==
% Algorithm used to find the best plan in the KB

%\paddingTopAlgorithm{}
\begin{algorithm}
  \caption{Find best plan}
  \label{alg:findBestPlan}
  \begin{algorithmic}[1]
    \Input{Query execution plan file $QEPF$}
    \Output{Mapped resource for the plan, $mapRes$}
    \Function{findBestPlan}{ $QEPF$ }
      \State $rdf$ := $createRDF$( $QEPF$ )
      \State $sparql$ := transform the rdf file $rdf$ into SPARQL query
      \State $mapRes$ := query the KB using the $sparql$ and map the $rdf$ to the best plan resources
      \State \Return{$mapRes$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}
%\paddingBottomAlgorithm{}

==> algorithms/QEPtoRDF.tex <==
% Algorithm to transform the query execution plan (QEP)
% into a RDF model

%\paddingTopAlgorithm{}
\begin{algorithm}
  \caption{Mapping QEPs to RDF graphs}
  \label{alg:QEPtoRDF}
  \begin{algorithmic}[1]
    \Input{QEP files $QEPs$[ ]}
    \Output{QEP files represented as RDF graphs, $RDFGs$[ ]}
    \Function{createRDFs}{ $QEPs$[ ] }
    \ForEach{$QEP$ in QEPs[ ]}
      \State $i$ := 0
      \State $MODEL$ := parse the $QEP$ file and save the properties
      \State $RDFG$ := convert $MODEL$ into a RDF graph model \mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }\mbox{       }with JENA RDF API
      \State $RDFGs$[ $i$ ] := $RDFG$
      \State $i$ := $i$ + 1
    \EndFor
    \State \Return{$RDFGs$[ ]}
    \EndFunction
  \end{algorithmic}
\end{algorithm}
%\paddingBottomAlgorithm{}

==> algorithms/Ranker.tex <==
% Algorithm used to rank the plans
% based in some properties

%\paddingTopAlgorithm{}
\begin{algorithm}
  \caption{Rank Plans}
  \label{alg:rankPlans}
  \begin{algorithmic}[1]
    \Input{db2batch Files $BATCHs$[ ]}
    \Output{A json file containing the ranked plans, $RANKED$[ ]}
    \Function{rankPlans}{ $BATCHs$[ ] }
    \ForEach{$batchf$ in BATCHs[ ]}
      \State $extractedValues$ := extract the properties from the $batchf$
      \State $plansProps$.$append$( $extractedValues$ )
    \EndFor
    \State $clusturedPlans$ := cluster the plans in $plansProps$ by the elapse time
    \State $RANKED$[ ] := rank best cluster in $clusturedPlans$ 
    \State \Return{$RANKED$[ ] as JSON}
    \EndFunction
  \end{algorithmic}
\end{algorithm}
%\paddingBottomAlgorithm{}

==> algorithms/TransformPlan.tex <==
% Algorithm used to transform the current plan 
% into the best one found in the KB

%\paddingTopAlgorithm{}
\begin{algorithm}
  \caption{Transform plan}
  \label{alg:transformPlan}
  \begin{algorithmic}[1]
    \Input{Query execution plan file, $QEPF$}
    \Output{Guideline with optimal way to execute the query, $guid$}
    \Function{TransformPlan}{ $QEPF$ }
      \State $rdf$ := $createRDF$( $QEPF$ )
      \State $QEPFs$[ ] := generate list of sub QEPs
      \ForEach{$subQEP$ in QEPFs[ ]}
        \State $mapRes$ := $findBestPlan$( $subQEP$ )
        \State $QEPF$ := apply the changes in the resources mapped $mapRes$
      \EndFor
      \State $guid$ := generate guideline for the modified $QEPF$
      \State \Return{$guid$}
    \EndFunction
  \end{algorithmic}
\end{algorithm}
%\paddingBottomAlgorithm{}

==> sections/acknowledgment.tex <==
\section{Acknowledgments}

The authors would like to thank members of the IBM DB2 optimizer development team for their valuable feedback and guidance through the development of the \toolName{} system. Special thanks in particular to Ian Finlay.

==> sections/trademarks.tex <==
\iffalse %Commented out, and only included if space permitting
\section{Trademarks} \label{section:Trademarks}

IBM, the IBM logo, and ibm.com are trademarks or registered 
trademarks of International Business Machines Corp., registered 
in many jurisdictions worldwide. Other product and service names 
might be trademarks of IBM or other companies. A current list of 
IBM trademarks is available on the Web at "Copyright and 
trademark information" at www.ibm.com/legal/copytrade.shtml.
\fi
